CUDA-L2: Surpassing cuBLAS Performance for Matrix Multiplication through Reinforcement Learning

In this paper, we propose CUDA-L2, a system that combines large language models (LLMs) and reinforcement learning (RL) to automatically optimize Half-precision General Matrix Multiply (HGEMM) CUDA kernels. Using CUDA execution speed as the RL reward, CUDA-L2 automatically optimizes HGEMM kernels across 1,000 configurations. CUDA-L2 systematically outperforms major matmul baselines to date, from the widely-used torch.matmul to state-of-the-art Nvidia's closed-source libraries, i.e., cuBLAS, cuBLASLt. In offline mode, where kernels are executed consecutively without time intervals, CUDA-L2 yields +22.0% over torch.matmul on average; +19.2% over cuBLAS using the optimal layout configuration (normal-normal NN and transposed-normal TN); +16.8% over cuBLASLt-heuristic, which queries cuBLASLt library and selects the algorithm based on the heuristic's suggestion; and +11.4% over the most competitive cuBLASLt-AutoTuning model, which selects the fastest algorithm from up to 100 candidates from cuBLASLt's suggestions. In server mode, where kernels are executed at random intervals simulating real-time inference, the speedups further increase to +28.7%, +26.0%, +22.4%, and +15.9% for torch.matmul, cuBLAS, cuBLASLt-heuristic, and cuBLASLt-AutoTuning respectively. CUDA-L2 shows that even the most performance-critical, heavily-optimized kernels like HGEMM can be improved through LLM-guided RL automation by systematically exploring configuration spaces at scales impractical for humans. Project and code can be found at github.com/ornith-ai/CUDA-L2

==> header_style.tex <==
% 一次性加载 geometry，给出页边距和 \headheight
% 增加 headsep 来让第一页页眉和正文之间有更大间距
\usepackage[margin=3cm, headheight=50pt, headsep=0pt]{geometry}

\usepackage{graphicx}   % 插图
\usepackage{fancyhdr}   % 自定义页眉页脚

% ------- 页眉定义 -------
\pagestyle{fancy}       % 默认页眉样式
\fancyhf{}              % 清空

% 删除默认页面的横线
\renewcommand{\headrulewidth}{0pt}

\begin{comment}
% 左侧：logo + 项目名，可按需删掉 \textsc{}
\fancyhead[L]{%
  \raisebox{-0.25\height}{\includegraphics[height=20pt]{./header.png}}%
}

% 右侧放页码示例（可不要）
\fancyhead[R]{}

% (2) 横向"拉长"：把页眉区域往左右各伸出 2.5 cm
\fancyheadoffset[L]{0.2cm}
\fancyheadoffset[R]{0.2cm}
\end{comment}

% 让首页 (plain) 同样使用这种页眉
\fancypagestyle{plain}{%
  \fancyhf{}
  \fancyhead[L]{%
    % 方法1：通过添加 \vspace 来让页眉内容下移
    \vbox to 25pt{%
      \vfill
      \raisebox{25pt}{\includegraphics[height=25pt]{./header.png}}%
      \vfill
    }%
  }
  \fancyhead[R]{
  \vbox to 25pt{%
      \vfill
      \raisebox{25pt}{}
      \vfill
    }%
  }
  \renewcommand{\headrulewidth}{0.7pt}  % 保留第一页的横线
  \fancyheadoffset[L]{0cm}
  \fancyheadoffset[R]{0cm}
}

% 如果只想让第一页的页眉和正文间距更大，可以在文档开始处使用：
% \thispagestyle{plain}
% \vspace{20pt}  % 在第一页正文开始前添加额外空间
